Search for Supersymmetry in Trilepton Final States with the ATLAS Detector and the Alignment of the ATLAS Silicon Tracker

One of the main goals of the ATLAS detector at the LHC of CERN, a proton-proton collider with a nominal centre-of-mass energy of 14 TeV, is to search for New Physics beyond the Standard Model (BSM). A widely favoured BSM candidate is Supersymmetry (SUSY), which postulates a superpartner for each Standard Model particle. The first part of this thesis describes a strategy for an early discovery of SUSY using the trilepton signature, with a focus on gravity-mediated SUSY breaking, mSUGRA. The discovery potential for SUSY for the case where strongly interacting supersymmetric particles are very massive is critically investigated. A possible choice of triggers for L = 10-31cm-2s-1 is suggested by optimising the event yield at intermediate and final selection stages. A novel method to measure the rate of leptons from heavy flavour decays passing isolation requirements by isolating tt events in data is outlined. The task of the ATLAS silicon tracker is to track particles produced in proton-proton collisions in its centre, measuring their momenta and production vertices. The precise knowledge of the silicon tracker module positions and their orientation in space (alignment) down to some microns and fractions of a miliradian in the critical coordinates is of vital importance for large parts of the ambitious ATLAS physics program. In the second part of the thesis, the alignment of the ATLAS silicon tracker using the Robust Alignment algorithm and particle tracks is described. The algorithm is applied to align end-cap A of the pixel detector using cosmic ray particle tracks recorded during its on-surface commissioning in 2006. Finally, about 2M cosmic ray tracks collected by ATLAS in situ in autumn 2008 are utilised to provide a coherent alignment of the entire silicon tracker with the Robust Alignment algorithm.

==> Bibliography/Bibliography.tex <==
\cleardoublepage

\addcontentsline{toc}{chapter}{Bibliography}

\baselineskip=3ex

\bibliographystyle{thesis}

\pagestyle{myheadings}
\markboth{Bibliography}{Bibliography}

\bibliography{references}



==> Introduction/Introduction.tex <==
%\pagenumbering{arabic}
% \setcounter{page}{1}
\begin{quote}
\textit{By convention sweet, by convention bitter, by convention hot, by convention cold, by convention colour: but in
reality atoms and void.}\begin{flushright}\footnotesize{Democritus, V-IV century b.C.}\end{flushright}
\end{quote}

For generations, Mankind is looking for answers on how our world is organised and what governs it in order to understand who we are by analysing \textit{our} reflection of the world. Evidence of ancestral cults indicating this continuous strive for explanations can be traced back to times as early as several tens of thousands of years ago. 
% It is remarkable that these dark ages of Mankind's birth were combined with the beginnings of the empirical observation of the surrounding environment.

A milestone to our modern view of the world was placed by Greek philosophers more than 3000 years ago. Besides bringing the idea of empiricism to a higher level, they contributed another essential element to Science as we know it today -- strict logic. An excellent example is the citation of Democritus above, who anticipated the main idea of Elementary Particle Physics by introducing the concept of ``the indivisible'' -- ``$\alpha\tau o\mu o\varsigma$'' from the observation that stepstones would be abraded in not visible, infinitely small pieces.

This approach was carried to a scientific level by (post-) renaissance philosophers.
% or, as they were called, \textit{thinkers}, for example by Goethe, who besides his poetic oeuvre had also some articles published on the origin of color ("Farbenlehre"). 
For the first time experiments were \textit{in\-ten\-tionally} and systematically designed to probe Nature. A milestone for the change of this paradigm is the works of Galileo. For instance, he derived the acceleration law $s=a/2\cdot t^2$ by measuring the acceleration due to Earth's gravitation using inclined surfaces and pendulums.

This naturally grown scientific approach has drastically changed our view of the world and our view of ourselves over the last millennia. The advancements of Science culminated in the great discoveries of the XX century, like the Theory of Relativity, Quantum Mechanics, the discovery of the role of the DNA, the ongoing investigation of the genome, and the understanding of the history of the Universe to name a few.

% However, besides the crucial breakthroughs listed above the most intriguing question still remains: what are the most elementary building blocks our world is made of? Elementary Particle Physics attempts to answer this question. Of course, there are no final answers and, luckily, never will be. But now we have all tools in place to make another step in the search for them: over the XX-th century the so-called Standard Model of Elementary Particle Physics has emerged \cite{bib:weinberg, bib:glashow, bib:salam,bib:gross, bib:politzer, bib:gell-mann,bib:higgs}, which serves us tremendously well in interpreting experimental findings; on the other hand in the beginning of the 90-ies the Tevatron, the world's most powerful proton anti-proton collider with a center-of-mass energy of $\sqrt s=1.96\,$TeV, was launched.
% 
However, besides the crucial breakthroughs listed above the most intriguing question still remains: what are the most elementary building blocks our world is made of? Elementary Particle Physics attempts to answer this question. Of course, there is no final answer and, fortunately, never will be. Over the XX-th century the so-called Standard Model of Elementary Particle Physics has emerged \cite{bib:weinberg, bib:glashow, bib:salam,bib:gross, bib:politzer, bib:gell-mann,bib:higgs}, which serves us tremendously well in interpreting experimental findings. In the beginning of the 90's the Tevatron, the world's most powerful proton anti-proton collider with a centre-mass energy of $\sqrt s=1.8\,$TeV, was launched. Its both experiments, \Dzero\ and CDF, are testing the validity of the Standard Model at this ever higher energy range and looking for New Physics. With success. The Tevatron's Run I culminated in the the discovery of the top quark in 1995 by \Dzero\ and CDF collaborations \cite{bib:top_discovery_d0, bib:top_discovery_cdf}. In fact, the top quark is the most recently discovered particle with the exception of the tau neutrino. The existence of the top quark was predicted in 1977 as the electroweak isospin partner of the bottom quark. Its mass, being the subject of this thesis, could be inferred from fits to electroweak precision data using theoretical input from the Standard Model. Finally, the prediction was confirmed by the discovery and direct measurement in 1995 \cite{bib:top_discovery_d0, bib:top_discovery_cdf} at the Tevatron.

The top quark is utterly interesting for a variety of reasons. The most intriguing one is risen by its high mass of $172.3\pm3.3\,$GeV \cite{bib:world_average}: is there a possible connection to the mechanism of the Spontaneous Symmetry Breaking? In the Standard Model, this mechanism is responsible for the masses of elementary particles. Canonically, Spontaneous Symmetry Breaking is incorporated in the Standard Model by introducing a scalar Higgs field with the Higgs boson being the excitation eigenstate of it \cite{bib:higgs}. Understanding the high mass of the top quark might yield new insights into Spontaneous Symmetry Breaking. The coupling of the Higgs field is strongest for the top quark together with the $\mathscr O(100{\rm \,GeV})$ heavy $W^\pm$, $Z$ bosons, compared to other elementary particles. In fact, their masses and the mass of the Higgs boson, which still remains to be found, are important parameters of the Standard Model and are connected to each other. This is why their precision measurement is so important and might reveal some New Physics. Furthermore, the high top quark mass results in an extremely short life time of $\tau\simeq0.5\times10^{-24}\,$s, which makes the formation of bound states impossible. Therefore, the information about its quantum numbers, for instance the spin, does not get lost and can be measured \cite{bib:spin_christian}. All this makes the top quark the hottest Elementary Particle Physics topic of our time.

At the Tevatron, the top quarks are dominantly produced in pairs. Within the Standard Model, there are 3 decay channels for a top anti-top pair. The subject of this thesis is the measurement of the top quark mass in the so-called dilepton channel, which is characterised by two bottom quarks and two leptons together with the corresponding neutrinos from $W$-boson decay in the final state. Despite the low branching ratio, the dilepton channel is highly important due to its low background and low systematics. It offers a possibility to test the Standard Model and could reveal New Physics, which cannot be seen in other channels. The presented analysis is based on the so-called Neutrino Weighting algorithm combined with the Maximum Method for the top mass extraction and was presented as a \Dzero\ preliminary at the ICHEP 2006 conference~\cite{bib:nwt_p17_conf,bib:nwt_p17_ana}. %In fact, it is the first dilepton top quark mass analysis at \Dzero\ with a smooth likelihood function without any systematic error due to fit uncertainties.

This Diploma thesis is organised as follows:
\begin{itemize}
	\item \textsc{Theoretical Aspects} relevant for this analysis covered in Chap.~\ref{chp:theory};
	\item The \textsc{Experimental Setup} -- the Tevatron and the \Dzero\ detector -- is described in Chap.~\ref{chp:setup};
	\item \textsc{The Analysed Dataset} and the selection criteria applied are explained in Chap.~\ref{chp:dataset};
	\item \textsc{The Neutrino Weighting Method} for inferring the top mass is described in Chap.~\ref{chp:nuwt};
	\item \textsc{The Maximum Method for the Top Quark Mass Extraction} is presented in Chap.~\ref{chp:maximum};
	\item \textsc{Testing the Maximum Method with Pseudo-Experiments} can be found in Chap.~\ref{chp:ensemble};
	\item \textsc{Results} found in all dileptonic channels of the \pbsmall\ dataset and in the \emu\ channel of the \pbbig\ dataset are presented in Chap.~\ref{chp:results};
	\item The \textsc{Systematic Uncertainties} are evaluated in Chap.~\ref{chp:systematics};
	\item \textsc{Conclusion} and \textsc{outlook} from the findings of this analysis are drawn in Chap.~\ref{chp:conclusion}~and~\ref{chp:outlook}.
\end{itemize}


% For generations, mankind is looking for answers on how the world we are living is built, and what governs it.
% Evidence of ancestral cults indicating this continuos strive for explanations can be traced back to times as early as
% several tens of thousands years ago. This was continued on a more advanced level by Greek philosophers before our era,
% for example Demokrit, %a defendant of the *** school, 
% who is cited above. This approach was carried to a scientific
% level by (post-) renaissance philosophers or, as they were called, \textit{thinkers}, for example by Goethe, who is
% mostly known for his poetic oeuvre but had also some articles published on the origin of color ("Farbenlehre"). This was
% enhanced by a scientific approach towards the experiment as we know it today, which is intentionally designed to probe
% the nature. A milestone for the change of this paradigm might be defined as the measurement of the acceleration by the
% gravitational force of the earth in fall experiments from the tower of Pisa using human heart beat rate for time
% measurement by Galileo Galilei. ...


==> RA/RobustAlignL1L2L3.tex <==
\include{Style}

\begin{document}

\section{Track Based Alignment}
\subsection{Alignment with Overlap Residuals}

In the following, the expression to calculate alignment corrections from residuals and overlap residuals will be introduced. Beforehand, however, a few definitions need to be made:
\begin{itemize}
 \item Capitalised variables stand for coordinates in the global ATLAS frame, small variables for the local module frame.
 \item Track-hit residuals in $\zeta$ are denoted as $r_{\zeta}\equiv\qhit_\zeta-\qtrk_\zeta$, where $\zeta=x,y$.
 \item The uncertainty on residuals is canonically defined as the estimator of the uncertainty on the mean, that is $\delta r_\zeta=\sigma(r_\zeta)/\sqrt{n_\zeta}$, where $\sigma(r_\zeta)$ is the standard deviation of $r_\zeta$, and $n_\zeta$ is the number of residuals collected by the respective module.
 \item Overlap residuals occur in the region where two modules have a geometrical overlap when a track produces hits in two neighbouring modules with identifiers $i$ and $i$+1 in the same layer. Depending on whether the overlap occurs with a neighbour in $\Phi$ or $\eta$, we speak about an overlap residual of $x$ or $y$ type, respectively. Naturally, an overlap residual can have two measurement directions: $x$ and $y$. Considering this, we denote overlap residuals as $o_{\zeta\xi}$, where $\zeta$ stands for the measurement direction, and $\xi$ defines the type of overlap.
 \item Whenever there is an overlap residual between two modules with $\Phi$- or $\eta$-identifiers $i$ and $i$+1, the overlap is assigned to the one with the larger identifier $i$+1. Thus we have for example $o_{\zeta\xi}^i=r_\zeta^i-r_\zeta^{i-1}$. Detector rings are circular, and therefore the module with a $\Phi$-identifier $i=0$ is assigned its overlap residual with the last module in the ring, i.e. the one with the largest $\Phi$-identifier.
 \item Similarly to the case of residuals, the uncertainty on overlap residuals is defined as $\delta o_{\zeta\xi}=\sigma(o_{\zeta\xi})/\sqrt{n_{\zeta\xi}}$, where $\sigma(o_{\zeta\xi})$ is the standard deviation of $o_{\zeta\xi}$, and $n_{\zeta\xi}$ is the number of overlap residuals collected in the overlap region of two respective modules.
\end{itemize}

\begin{figure}[b]
\begin{center}
\includegraphics[width=10.5cm,clip=true]{figures/ovres.eps2}\qquad
\end{center}
\caption{\label{fig:ovres}
Overlap residuals: situation as it is in reality {\bf (a)} and as seen by the reconstruction {\bf (b)}.
}
\end{figure}%\nopagebreak[5]



To verify that the sign convention is correct, we need to consider that the $\Phi$ direction and thus the direction of increasing $\Phi$-identifiers of modules conicide with the positive $x$ direction of each module. Thus, for a correction $c_{xx}^i$ for the module $i$ from $o_{xx}^{i}$, $o_{xx}^{i+1}$ overlap residuals we use the expression:
\begin{equation}
  \label{eqn:c_xx}
  c_{xx}^i=\frac12\cdot\fdampover\cdot 
           \frac{
   - \frac{\bra o_{xx}^i\ket}{(\delta o_{xx}^i)^2} 
   + \frac{\bra o_{xx}^{i+1}\ket}{(\delta o_{xx}^{i+1})^2}
                }{ 
     \frac{1}{(\delta o_{xx}^{i})^2} 
   + \frac{1}{(\delta o_{xx}^{i+1})^2}
                }
  \,.
\end{equation}
As is evident from the factor \oneOverTwo{} in the formula, corrections resulting from the overlap $o_{xx}^i$ are equally shared between modules $i$--1 and $i$. \fdampover{} is a tuning factor typically in the range of $[0.5,\,1]$, which is supposed to correct for a slight overcompensations of misalignments when $\fdampover\equiv1$, resulting in a sub-optimal conversion. A value of $\fdampover\simeq0.7$ was found to be a good choice.

The error on the $c_{xx}^i$ correction, $\delta c_{xx}^i$, is defined as:
\begin{equation}
  \label{eqn:dc_xx}
  \delta c_{xx}^i=\left\{
     \frac{1}{(\oneOverSqrt\cdot\delta o_{xx}^{i})^2} 
   + \frac{1}{(\oneOverSqrt\cdot\delta o_{xx}^{i+1})^2} 
                  \right\}^{-\oneOverTwo}
\end{equation}
in accordance to Eqn.~\ref{eqn:c_xx}. The only difference to what Eqn.~\ref{eqn:dc_xx} suggests, is an additional factor of \oneOverSqrt{}, which accounts for the fact, that corrections are shared between two neighbouring modules. On the contrary, using the full error $\delta o_{xx}$ would imply a larger uncertainty on overlap residuals when considering all the modules. $\fdampover$, being a tuning factor, is not considered in the error calculation\footnote{The appropriateness of this can be seen by considering (an unreasonably) small value of $\fdampover \ll 1$, which would result in very small uncertainties on the correction $c_{xx}$.}.

Taking into account Eqn.~\ref{eqn:c_xx} for corrections $c_{xx}^i$ resulting from $o_{xx}^{i,i+1}$ overlap residuals, the corresponding expression for $c_{xy}^j$ from $o_{xy}^{j,j+1}$, where $i,j$ are the $\Phi$- and $\eta$-identifiers of the module considered, and the corrections from plain residuals $c_x^i$, we can construct the full expression for the module corrections:
\begin{equation}
  \label{eqn:c_xtotal}
  c_{x,\rm total}^i= \frac{ 
   - \frac{\bra r_x^i\ket}{(\delta r_x^i)^2}
   + \frac12\cdot\fdampover\cdot\left\{
   - \frac{\bra o_{xx}^i\ket}{(\oneOverSqrt\cdot\delta o_{xx}^i)^2} 
   + \frac{\bra o_{xx}^{i+1}\ket}{(\oneOverSqrt\cdot\delta o_{xx}^{i+1})^2}
   - \frac{\bra o_{xy}^j\ket}{(\oneOverSqrt\cdot\delta o_{xy}^j)^2} 
   + \frac{\bra o_{xy}^{j+1}\ket}{(\oneOverSqrt\cdot\delta o_{xy}^{j+1})^2}
     \right\}
                          }{ 
     \frac{1}{(\delta r_x^i)^2}
   + \frac{1}{(\oneOverSqrt\cdot\delta o_{xx}^{i})^2} 
   + \frac{1}{(\oneOverSqrt\cdot\delta o_{xx}^{i+1})^2}
   + \frac{1}{(\oneOverSqrt\cdot\delta o_{xy}^{j})^2} 
   + \frac{1}{(\oneOverSqrt\cdot\delta o_{xy}^{j+1})^2}
                          }
  \,.
\end{equation}
Consequently, the error on $c_{x,\rm total}^i$ is given by:
\begin{equation}
  \label{eqn:dc_xtotal}
  \delta c_{x,\rm total}^i=\left\{ 
     \frac{1}{(\delta r_x^i)^2}
   + \frac{1}{(\oneOverSqrt\cdot\delta o_{xx}^{i})^2} 
   + \frac{1}{(\oneOverSqrt\cdot\delta o_{xx}^{i+1})^2}
   + \frac{1}{(\oneOverSqrt\cdot\delta o_{xy}^{j})^2} 
   + \frac{1}{(\oneOverSqrt\cdot\delta o_{xy}^{j+1})^2}
                           \right\}^{-\oneOverTwo}
  \,.
\end{equation}

%\begin{thebibliography}{99}
% \bibitem{bib:RobustAlignment}
% F.~Heinemann, ``Track Based Alignment of the ATLAS Silicon Detectors with the Robust Alignment Algorithm'', ATL-INDET-PUB-2007-011; F. Heinemann, PhD Thesis, Univ. of Oxford, in preparation for 2007; D. Hindson, PhD Thesis, Univ. of Oxford, 2004.
%\end{thebibliography}

\end{document}


==> Theory/Top.tex <==
In the following, a brief overview of Top Physics at the Tevatron shall be given. The production of the top quark in \ttbar\ pairs is discussed. Thereafter, the properties of the top quark are covered. A more detailed review can be found in~\cite{bib:arnulf_review}. A special focus is placed on the relevance of a precision measurement of the top quark mass, being the subject of this thesis.

\subsection{Top Anti-Top Pair Production}
The top quark was discovered as lately as in 1995 by the \Dzero\ and CDF collaborations \cite{bib:top_discovery_d0, bib:top_discovery_cdf} after its prediction as the electroweak partner of the bottom quark in 1977. In fact, the top quark is the most recently discovered elementary particle, up to the $\tau$-neutrino.

At the Tevatron, the top quark production has so far been observed via the strong interaction in \ttbar\ pairs: $q\bar q\rightarrow \ttbar$ which accounts for 85\% (90\%) of the total cross section of the process, and $gg\rightarrow \ttbar$ contributing with 15\% (10\%). The numbers in parentheses give the corresponding numbers for Tevatron's Run I\footnote{for more details on the Tevatron, its two collider experiments \Dzero\ and CDF, the Run I and II refer to Chap.~\ref{chp:setup}.} at $\sqrt s=1.8$\,GeV. For the Large Hadron Collider, relative contributions of 10 and 90 percent are predicted, respectively. In Fig.~\ref{fig:feyn_ttbar_prod} the corresponding tree level production diagrams are shown.

\begin{figure}
\centering
\includegraphics[width=0.6\textwidth]{Theory/fig/topprod.eps}
\caption{\small\label{fig:feyn_ttbar_prod}
Tree level Feynman diagrams for \ttbar\ production at the Tevatron: quark anti-quark annihilation (85\%) in the top row and gluon-gluon fusion (15\%) in the $t$, $u$, and the $s$ channel going from left to right in the bottom row.
}
\end{figure}

The total cross section for the strong \ttbar\ production is approximately $\sigma_{\ttbar}\simeq7$\,pb. A summary of the cross section predicted and measured in Run I and II per-experiment is given in Tab.~\ref{tab:ttbar_Xsec}.

\begin{table}
\centering
\begin{tabular}{llll}
\hline
$\sigma_{\ttbar}$ [pb]	& \Dzero			& CDF				& Theory\\
\hline\hline
Run I			& $5.7\pm1.6$			& $6.5~^{+~1.7}_{-~1.4}$	& $4.5-5.7$\\
Run II			& $7.1~^{+~1.9}_{-~1.7}$	& $7.3\pm0.9$			& $5.8-7.4$\\
\hline
\end{tabular}
\caption{\small\label{tab:ttbar_Xsec}
The total cross section for the strong \ttbar\ production measured by the \Dzero\ and CDF experiments in Run I and II of the Tevatron, as summarised in~\cite{bib:pdg2004}. The Run II figures include published results only. The theoretical prediction was calculated in~\cite{bib:kidonakis1, bib:kidonakis2} for a top quark mass of $\mtop=175\,$GeV.
}
\end{table}

The cross section for the top quark production is determined by the centre-of-momentum energy of the participating (anti-) quarks and gluons. This energy depends on the one hand on the centre-of-mass energy $\sqrt s$ of the $p\bar p$ system, and on the other hand on the fraction of the total proton momentum $x_i$ carried by the $i$-th participating (anti-) quark or gluon in the parton model. With $p_p$, $p_{\bar p}$ being the 4-momenta of the proton and the anti-proton, the effectively available centre-of-mass energy $\sqrt{\tilde s}$ becomes:
	\[\tilde s=(x_1p_p+x_2p_{\bar p})^2\stackrel{m_p\rightarrow0}{\simeq}2\cdot x_1x_2\cdot p_pp_{\bar p}=x_1x_2\cdot s\,.\]
If for the sake of the argument $x_1\equiv x_2$ and a top quark mass of $\mtop=175$\,GeV are assumed, for the production of a \ttbar\ pair a minimum momentum fraction $x_{\rm min}\simeq2\cdot\mtop/{\sqrt s}=0.18$ is required. 

In Fig.~\ref{fig:cteq} (left) the Parton Distribution Function (PDF) set is shown in version CTEQ5L for the various parton flavours~\cite{bib:cteq5}. These PDF's are used with the \pbsmall\ dataset and the \texttt{p14} version of \Dzero\ software (Chap.~\ref{chp:dataset}). The parton distribution function $f(x)$ gives via $xf(x){\rm d}x$ the probability for a parton to carry a momentum fraction between $x$ and $x+{\rm d}x$. 

\begin{figure}
\centering
\includegraphics[width=0.55\textwidth]{Theory/fig/CTEQ5.eps}
\includegraphics[width=0.415\textwidth,clip=]{Theory/fig/cs1960plotdpf04.eps}
\caption{\small\label{fig:cteq}
The Parton Distribution Function (PDF) set CTEQ5L at the scale $Q^2=175\,$GeV, as determined by the CTEQ collaboration \cite{bib:cteq5} is shown on the left hand side. The minimum momentum fraction $x_{\rm min}$  bands defined in the text are marked as vertical lines for Tevatron and LHC centre-of-mass energies. On the right hand side the dependence of the total \ttbar\ cross section on the top quark mass as in \cite{bib:kidonakis1, bib:kidonakis2} is shown.
}
\end{figure}

Besides the dependence on the centre-of-mass energy available, the \ttbar\ production cross section depends on the top quark mass. This relation is depicted in Fig.~\ref{fig:cteq} (right), as calculated in \cite{bib:kidonakis1, bib:kidonakis2}.

\subsubsection{The Dilepton Decay Channel}
According to the Standard Model and assuming 3 quark generations, the top quark predominantly decays into its weak interaction partner, the bottom quark, with a branching ratio $f_{\rm BR}(t\rightarrow Wb)>0.998$ \cite{bib:pdg2004}. This is due to the fact that $|V_{tb}|\simeq1$, as follows from the unitarity of the CKM matrix and the measurement of its other elements. Each of the $W$-bosons can subsequently decay leptonically ($f_{\rm BR}^e=10.72\pm0.16$, $f_{\rm BR}^\mu=10.57\pm0.22$, $f_{\rm BR}^\tau=10.74\pm0.27$; 1/9 each at Born level, all numbers are from \cite{bib:pdg2004}) or hadronically ($f_{\rm BR}^{\rm hadrons}=67.96\pm0.35\simeq3\cdot2/9$ at Born level, where the number 3 accounts for the number of strong colour charges and 2 is the number of quark generations available for $W$ decay regarding energy conservation). This defines three decay channels for a \ttbar\ pair: the dileptonic channel, being the subject of this thesis, where both $W$-bosons decay leptonically, the semileptonic channel where one $W$ decays leptonically and the other hadronically, and the all-jets channel, where both $W$-bosons decay hadronically.

\begin{figure}
\centering
\includegraphics[height=0.35\textwidth]{Theory/fig/top_pair_decay_channels.eps}\qquad
\includegraphics[height=0.32\textwidth]{Theory/fig/top_decay_mk00.eps}
\caption{\small\label{fig:pie_chart}
On the left hand side a summary of the decay subchannels of a \ttbar\ pair is given. The right hand side displays the relative contributions at Born level. The $\tau$-inclusive contribution of the dilepton channel is approximately 5\%.
}
\end{figure}

The decay channels of a \ttbar\ pair are listed schematically on the left hand side of Fig.~\ref{fig:pie_chart}, their relative contributions are shown in a pie chart on the right hand side. However, the $\tau$-leptons have a short life time and are not detected directly. Therefore, the dilepton channel is understood to be defined with either 2 electrons, 2 muons, or an electron and a muon in the final state. These final states include leptonic decays of the $\tau$-lepton: $\tau\rightarrow e$ ($f_{\rm BR}=17.84\pm0.06$) and $\tau\rightarrow\mu$ ($f_{\rm BR}=17.36\pm0.06$). Taking this into account, the branching ratios in the dilepton channel are:
\begin{center}
\begin{tabular}{llr}
\hline
Channel	& Process (incl.)					& $f_{\rm BR}$ [\%], from \cite{bib:pdg2004} \\
\hline\hline
\emu:	& $\ttbar\rightarrow e^{\pm}\mu^{\mp}b\bar b\nu's$ 	& $3.16\pm0.06$ \\
\ee:	& $\ttbar\rightarrow e^{+}e^{-}b\bar b\nu's$ 		& $1.58\pm0.03$ \\
\mumu:	& $\ttbar\rightarrow \mu^{+}\mu^{-}b\bar b\nu's$ 	& $1.57\pm0.03$ \\
\hline
\end{tabular}
\end{center}
The total contribution of the dilepton channel including leptonic $\tau$-decays is 6.3\%. However, the dilepton channel is very important. Due to the two leptons and fewer jets in the final state, it potentially has the lowest systematic error of all \ttbar\ decay channels and will provide a top quark mass measurement of a similar precision as the semileptonic channel once a certain integrated luminosity is collected. Further, New Physics which is not visible in other decay channels may be found in the dilepton channel. Additionally, precision measurements can be made in the dilepton channel to test the Standard Model.
% \footnote{In fact, the \Dzero\ ($\mtop=168.4\pm12.8$\,GeV) and CDF ($\mtop=167.4\pm11.4$\,GeV) measurements of the top quark mass using the dilepton channel made in Run I as well as the CDF ($\mtop=165.2\pm7.0$\,GeV) measurement in Run II are all $\sim7\,$GeV lower than the combined world average value of $\mtop=174.2\pm3.3$\,GeV \cite{bib:world_average}.}.

The basic signature of a dileptonic \ttbar\ event is evident from the tree level Feynman diagram in Fig.~\ref{fig:feyn_ttbar_dilepton}, which represents the simplest decay scenario without any $\tau$-leptons or any initial/final state radiation: 
	\[q\bar q,\,gg\rightarrow\ttbar+X\rightarrow l^-\bar\nu\bar bl^+\nu b+\tilde X\,,\]
where $X,\tilde X$ are any additionally produced particles. Thus, as a signature, one expects 2 leptons and 2 $b$-jets. All 4 physics objects should have a high $p_T$ and be central (i.e. have a low $|\eta|$) due to the high mass of a \ttbar\ pair and the fact that its rest frame almost coincides with the rest frame of the detector. This can be seen from steeply falling parton distribution functions, which makes equal momentum fractions for both partons probable. Due to a $b$-jet fragmentation as well as possible initial and final state radiation the 2 jet bin is understood to be inclusive. Further, large \met\ values are expected due to 2 or more neutrinos. The background processes to mimic this signature are discussed in Sec.~\ref{sec:background}.

\begin{figure}
\centering
\includegraphics[width=0.6\textwidth]{Theory/fig/feyn_dilepton.eps}
\caption{\small\label{fig:feyn_ttbar_dilepton}
Tree level Feynman diagram for the simplest \ttbar\ decay scenario into the dilepton channel.
}
\end{figure}

\subsection{Properties of the Top Quark}
\subsubsection{Top Quark Mass}
The top quark mass is a fundamental parameter of the Standard Model. The importance of its precision measurement will be detailed in the following. Currently, the world average top quark mass including preliminary results is \cite{bib:world_average}:
\begin{eqnarray*}
\mtop^{\rm publ.+prel.} 			&=& 171.4 \pm 2.1\,{\rm GeV} (\rm stat.+syst.)\,.
\end{eqnarray*}

Before the direct measurement by both Tevatron collider experiments in 1995~\cite{bib:top_discovery_d0, bib:top_discovery_cdf}, the top quark mass has been inferred using the Standard Model prediction manifest in radiative corrections to the $W$-boson mass with electroweak precision data. The theoretical background is briefly outlined in the following. In Fig.~\ref{fig:mtop_vs_time} the evolution of the top quark mass is shown \cite{bib:mtop_vs_time}.

\begin{figure}
\centering
\includegraphics[width=0.8\textwidth]{Theory/fig/mtop_vs_time}
\caption{\small\label{fig:mtop_vs_time}
Evolution of the top quark mass prediction from electroweak precision data (\textcolor{green}{$\bullet$}) and direct measurements 
(CDF: \textcolor{blue}{$\blacktriangle$}, \Dzero: \textcolor{red}{$\blacktriangledown$}) with time. The world average from direct measurement is shown as \textcolor{magenta}{$\blacksquare$}. Furthermore, the lower bounds from hadron colliders (dashed lines) and $e^{+}e^{-}$ colliders (solid line) are presented. (Updated: Sept. 2005 by Chris Quigg from \cite{bib:mtop_vs_time}).
}
\end{figure}

To leading order, the electroweak interaction depends solely on a set of 3 independent parameters. Conveniently, these three parameters are chosen to be the electromagnetic coupling constant $\alpha$ which is precisely measured in low-energy experiments, the Fermi constant $G_F$ determined in weak decay experiments, and the mass of the $Z$ boson $m_Z$ measured at LEP with a high precision. With these parameters, the mass of the $W$ boson can be expressed as:
\begin{equation}\label{eqn:m_w_lo}
	m_W^2=\frac{\frac{\pi \alpha}{\sqrt{2}G_{F}}} {\sin^2(\theta_W)}\,,
\end{equation}
where $\sin^2(\theta_W):=1-\frac{m_W^2}{m_Z^2}$ defines the Weinberg angle $\theta_W$. 

With loop corrections in next-to-leading order included, contribution to the self-energy of the $W$-boson stemming from the virtual top quark and the Higgs boson are to be included, and Eqn.~\ref{eqn:m_w_lo} modifies to:
\begin{equation*}
	m_W^2=\frac{\frac{\pi \alpha}{\sqrt{2}G_{F}}} {\sin^2(\theta_W)(1-\Delta r)}\,,
\end{equation*}
where $\Delta r$ represents the next-to-leading order corrections. These corrections to the $W$ and $Z$ boson mass originate from the following Feynman diagrams:\\
	\hspace*{0.2\textwidth}\includegraphics[width=0.6\textwidth]{Theory/fig/toploops.eps}\\
and yield:
\begin{equation}\label{eqn:dr_top}
	(\Delta r)_{\rm top} \simeq -\frac{3G_{F}}{8\sqrt{2}\pi^{2} \tan^2\theta_{W}}\cdot
	%\frac1{\mtop^{2}}\,.
	\mtop^{2}\,.
\end{equation}
For the Higgs boson, the virtual corrections\\
	\hspace*{0.2\textwidth}\includegraphics[width=0.6\textwidth]{Theory/fig/higgsloops_00.eps}\\
result in logarithmic contributions due to the different loop type which accounts for the scalar nature of the Higgs boson. Numerically, the correction is:
\begin{equation}\label{eqn:dr_higgs}
	(\Delta r)_{h} \simeq \frac{11G_{F}m_{Z}^{2}\cos^2\theta_{W}}{24\sqrt{2}\pi^{2}}
                                      \cdot\ln\frac{m_{h}^{2}}{m_{Z}^{2}}\,.
\end{equation}

\begin{figure}
\centering
\includegraphics[width=0.6\textwidth]{Theory/fig/lepew_fit_1992.eps}
\caption{\small\label{fig:mtop_chi2_lep}
The \chisq\ of the Standard Model fit to the electroweak precision measurements as a function of the top quark mass using the data of LEP I only (left) and data from LEP, neutrino and hadron collider experiments (right)~\cite{bib:mtop_chi2}. The curves are displayed for 3 Higgs boson masses: 50\,GeV (the limit from direct searches at LEP I), 300\,GeV, and 1000\,GeV (the upper limit allowed by the theoretical framework of the Standard Model). The minima of these curves are close together due to the logarithmic dependence on the Higgs mass, whereas the top quark mass enters quadratically.
}
\end{figure}

It is important to stress, that the contribution of Eqn.~\ref{eqn:dr_top} is quadratic, whereas the contribution of Eqn.~\ref{eqn:dr_higgs} is logarithmic and thus rather weak. Therefore, the top quark mass contributes much stronger to the self-energy of weak bosons than the Higgs boson. This instance was successfully used to predict the top quark mass using electroweak precision measurements, as shown in Fig.~\ref{fig:mtop_chi2_lep}~\cite{bib:mtop_chi2}. It is remarkable, that in 1992, 3 years before the discovery of the top quark, its mass was predicted with a relatively high precision and fully confirmed later. %This fact was interpreted as a strong argument pro the radiative approach of the Standard Model.
The most recent indirect measurements of the top quark mass yield \cite{bib:mtop_electroweak_new1,bib:mtop_electroweak_new2}:
\[
	\mtop=179.4~^{+12.1}_{-\phantom{1}9.2}\,{\rm GeV}\,,
\]
and are in a good agreement with the world average top quark mass.

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{Theory/fig_lep/s06_mt_mw_contours.eps}
\includegraphics[width=0.4\textwidth]{Theory/fig_lep/s06_blueband.eps}
\caption{\small\label{fig:mw_vs_mtop}
The left hand side shows the lines of constant Higgs mass for 114, 300, and 1000\,GeV in the $W$-boson mass versus top quark mass plane. Further, as a dotted ellipse, the 68\% confidence level for the direct measurements of $m_W$ and $\mtop$ is shown. The solid ellipse is the 68\% confidence level for the indirect measurement of $m_W$ and \mtop\ from precision electroweak data. The right hand side demostrates the so-called Blueband plot, showing the Higgs boson mass as determined from electroweak precision data together with the 95\% confidence level lower limit from direct searches. The yellow region marks Higgs masses exclueded with LEP direct search results~\cite{bib:higgs_lep2}. Both plots are from \cite{bib:mtop_electroweak_new3}.
}
\end{figure}

Now, after the discovery of the top quark and the precision measurement of its mass (which is constrained to 1.2\% regarding the world average top quark mass including published and preliminary results~\cite{bib:world_average}), the mass of the elusive Higgs boson can be predicted from the precision measurement of the $W$-boson mass. For the Run II of the Tevatron, for the the $W$-boson mass an uncertainty of 20\,MeV is expected. In terms of the projected uncertainty on the Higgs boson mass, this corresponds to an error on the top quark mass of $\sim$3\,GeV. This goal has already been overachieved. The left hand side of Fig.~\ref{fig:mw_vs_mtop} shows the $W$-boson mass versus top quark mass plane, with lines of constant Higgs boson masses at 114\,GeV (values of under 114.4\,GeV have been exclueded by LEP~\cite{bib:higgs_lep2}), 300\,GeV and 1000\,GeV (excluded as the limit of validity of the Standard Model). As a dotted ellipse the direct measurements of the top quark and $W$-boson mass are shown, the solid ellipse represents electroweak precision data results. It can be clearly seen that these measurements favor a light Higgs mass. The plot on the right hand side of Fig.~\ref{fig:mw_vs_mtop} shows the Higgs mass prediction from all electroweak precision data together with the 95\% confidence level lower limit from direct searches. This fit yields $85^{+39}_{-28}\,$GeV~\cite{bib:mtop_electroweak_new3} for the Higgs mass which is slightly below the limit excluded in the direct search for a Standard Model Higgs at LEP.

\subsubsection{The Decay Width of the Top Quark}
Due to its large mass, the top quark has a very short life time of $\tau_{\rm top}\simeq0.5\times10^{-24}\,$s or, alternatively, a decay width of $\Gamma_{\rm top}\simeq1.5\,$GeV \cite{bib:decay_width}. This makes the top quark an interesting study object, since it is the only known quark with a life time lower than the hadronisation time scale $\mathscr{O}(10^{-23}\,{\rm s})$, estimated by $\Lambda_{\rm QCD}^{-1}\simeq200^{-1}\,{\rm MeV}^{-1}$. This means that the top quark decays via the weak interaction before it hadronises and that no bound states like $t\bar q$ etc. can be formed. Therefore, by measuring the final state in the detector the physics properties of a ``naked'' quark can be studied for the first time in the history of Elementary Particle Physics. In particular, this is true for quantum numbers of the top quark like the spin.

\subsubsection{$W$-Helicity Measurements}
The preserved spin information of the top quark provides a unique possibility to verify the $V-A$ nature of the $Wtb$ coupling. As a fermion, the bottom quark must be left-handed in the massless limit, which forbids right-handedness for the W-boson: then the total angular momentum would be 3/2 in the top rest frame, whereas the Standard Model top quark has spin 1/2. Therefore, a measurement of the fraction $f_+$ of right-handed $W$-bosons is an important test of the Standard Model. For the fraction of longitudinally polarised $W$-bosons
\[
	f_0=\frac{\mtop^2/2m_W^2}{1+\mtop^2/2m_W^2}\simeq70\%
\]
according to the Standard Model. Various approaches are used at \Dzero\ and CDF to measure the fractions $f_0$, $f_+$, and $f_-$. The latest Run~II results are:\\\hspace*{0.3\textwidth}
\begin{tabular}{llll}
$f_+$ & $<$ & $0.24$ (95\% CL)		& (\Dzero, \cite{bib:d0_whel1,bib:d0_whel2})\\
$f_+$ & $<$ & $0.27$ (95\% CL)		& (CDF, \cite{bib:cdf_whel})\\
$f_0$ & $=$ & $0.74~^{+0.22}_{-0.34}$	& (CDF, \cite{bib:cdf_whel})\,.
\end{tabular}

\subsubsection{Spin Correlations of \ttbar\ Pairs}
Since the top quark decays before hadronisation due to its large mass, its spin is experimentally accessible. The beams at the Tevatron are not polarised. However, the spin information can be inferred from the correlation of the $t$ and the $\bar t$ in strong top pair production. For the dilepton channel, the relevant angular distribution of charged leptons coming from the top and the anti-top is
\[
	\frac{1}{\sigma}\frac{{\rm d}^2\sigma}{{\rm d}(\cos\theta_+){\rm d}(\cos\theta_-)}
	= \frac{1+\kappa\cdot\cos\theta_+\cos\theta_-}{4}\,,
\]
where $\theta_+$, $\theta_-$ are the angles of the charged leptons with respect to a particular quantisation axis in the top rest frame, at the Tevatron conveniently chosen to be the beamline axis. For a centre-of-mass energy of $\sqrt s=1.96\,$GeV ($\sqrt s=1.8\,$GeV), the correlation coefficient $\kappa$ is expected to be $\kappa\simeq93\%$ (88\%) \cite{bib:spin_christian,bib:pdg2004,bib:arnulf_review}. \Dzero\ has measured the spin correlation using dilepton events in Run~I~\cite{bib:spin_runi}, and found a weak preference for the Standard Model prediction. A limit of $\kappa>-0.25$ is quoted at 68\% confidence level. In Run II of the Tevatron, an observation of spin correlations is expected, and at \Dzero\ efforts are underway \cite{bib:spin_christian}.

\subsubsection{Electric Charge of the Top Quark}
The electric charge of the top quark is measured at the Tevatron in order to exclude a non-Standard Model quark $Q_4$ with a charge of $-4/3$ and the $Q_4\rightarrow W^-b$ decay mode. This $t$-$Q_4$ ambiguity is present at both Tevatron collider experiments, since the pairing of the $b$-quarks and the $W$-bosons is not determined in the strong top quark production $p\bar p\rightarrow\ttbar\rightarrow W^+W^-b\bar b$. Canonically, the charge of the top quark could be easily accessed at an $e^+e^-$ collider by measuring the ratio \linebreak[5] $R=\frac{e^+e^-\rightarrow\rm hadrons}{e^+e^-\rightarrow\mu^+\mu^-}$ below and above the top quark production threshold. At the Tevatron, different approaches have to be taken: either the charge of the decay products, or the photon radiation rate has to be determined in \ttbar\ events. So far, the top quark charge has been investigated by \Dzero\ only and the $Q_4$-scenario can be ruled out at 94\% level \cite{bib:top_charge}.

\section{Background Processes}\label{sec:background}
The main \textit{background physics processes} contributing in all three dileptonic channels are:
\begin{itemize}
        \item Drell-Yan: $Z/\gamma^*\rightarrow\tau\bar\tau\rightarrow l_1\bar\nu_{l_1}\bar l_2\nu_{l_2}$, where $l_i=e,\mu$, with two or more associated jets from initial or final state radiation.
        \item Di-boson production: $W^+W^-\rightarrow l_1\bar\nu_{l_1}\bar l_2\nu_{l_2}$, again with two associated jets. The yields for the $WZ$ and $ZZ$ processes are an order of magnitude lower \cite{bib:Xsec_p14_all, bib:Xsec_p14_arxiv}. Therefore, they are not considered in this analysis.
\end{itemize}
Due to the presence of neutrinos, the processes above contain real\footnote{``Real'' in this context refers to ``not faked''.} missing energy \met.

One has to consider, especially for the \ee~and \mumu~channels, another class of background events, the so-called \textit{instrumental background} events. These are physics processes where a physics object is mis-measured, for example \met, due to its finite resolution or mis-reconstruction.

The by far largest contribution to the instrumental background comes from $Z/\gamma^*\rightarrow e\bar e,\mu\bar\mu$ with associated jets.
The final yield of these processes is comparable to $Z/\gamma^*\rightarrow\tau\bar\tau$, since the low probability for a mis-measurement of the Gaussian distributed \met\ in $Z/\gamma^*\rightarrow e\bar e,\mu\bar\mu$ is compensated by a branching ratio of unity for $e\rightarrow e$, $\mu\rightarrow\mu$, whereas $\tau\rightarrow e=17.84\%$, $\tau\rightarrow\mu=17.36\%$ \cite{bib:pdg2004} for $Z/\gamma^*\rightarrow\tau\bar\tau$.

Another significant source of instrumental background in all 3 channels is the production of multijet final states (QCD multijet background). So for instance an electron can be faked by a $\pi^0$, and a secondary muon coming from within a jet can be isolated and thus survive the selection cuts due to mis-reconstruction.

% \subsubsection{CKM matrix element $|V_{tb}|$}
% \subsubsection{Single Top Production}
%   maybe?
% \subsection{Background Processes}
%  maybe later, in the chapter on the selection?


==> WeakMode/WeakMode.tex <==
Pawel's Siena proceedings: \cite{bib:procSiena}.

From Anthony:
\begin{verbatim}
> Hi Anthony,
> > 
> > this was REALLY quick! Thanks a lot for getting back to me so promptly!
> > Only a few weeks for you to enjoy CERN, and then back to Melbourne? Do you
> > need collision data to graduate? (with me cosmics were fine!)
> > 
> > See for my comments below, but beforehand could I ask you some questions to
> > understand your plots a bit better (sorry, some of them must sound really
> > silly, but my brain is a bit mushy from all the thesis typing...)
> > plot 1: 
> > - the right plot is labelled ?QoverPt/QoverPt, whereas all the other ones are
> > just ?X. I guess page 1 is then a typo?

No typo on page 1-- they were just normalised to somewhat remove the energy
dependence of the resolution.

> > plots 1-6: 
> > - these are for the Si-only tracks, right?
correct

> > - in the left plot, do you define the pull as value/sigma(value), where sigma
> > is the error? 
(Truth-Reco)/Reco Error

> > - in the right plot, what is ?X? it can't be the error, since negative. Is it
> > the bias? w/r/t what?
?X is just the residual between the Truth and the Reconstructed value (Units
are Atlas standard (mm and radians)).

> > plot 7 (for iter0) and 8 (for iter8):
> > - by comparing those two, I tend to conclude that the q.p_T bias we were
> > observing before is slightly overcorrected, since the slope changes?
> > plot 8 (for iter0):
> > - I see there is some q.p_T bias, which is opposite to the one seen in Si. I
> > don't understand why it's there: these are TRT segments which should be
> > independent from the Si and consequently unbiased in terms of q.p_T?

Ok basically I used a perfectly aligned TRT detector but had the SCT in the
curl geometry.  So you can see that even with TRT in the perfect geometry
(Iter0) the TRT segments have a PT bias caused by the misalignment between
the SCT and TRT.

This is then propagated to the SI geometry .. leading to the match biases.
Which is what you expect and actually show that the constraint is working
well.


I hope that clear things up

Cheer

Anthony
\end{verbatim}
******************
\begin{verbatim}
Absolutely no problem.  I have been revisiting this same stuff for my
thesis.

On 6/05/09 5:25 PM, "Oleg Brandt" <o.brandt@physics.ox.ac.uk> wrote:

> > Hi Anthony,
> > 
> > thanks a lot for your explanations, now everything makes sense!
> > 
> > Please bear with me -- I have two remaining questions...
> > 
> > Could you roughly explain the mechanism why TRT segments have a p_T bias? I
> > thought that TRT segments are reconstructed completely independently of the
> > Si, and therefore should not have any bias for a perfect TRT detector? Or are
> > these the TRT parts of the combined tracks?

We take Si+TRT tracks and snap off the TRT hits and refit them constraining
the Z0 and theta parameters to those obtained from Si+TRT track. Because the
TRT and SI start off with the outer layer of the SCT rotated wrt to the TRT
this puts a bias  on the momentum measurement and theta (very small but
measureable).  This bias in theta is then propagated through the whole
alignment process. Leading to the biased results you observe. I know it is a
bit a stretch to see this but this was the only way I could explain my
results and how you get a bias in the pT despite the perfect geometry.


>> >> Ok basically I used a perfectly aligned TRT detector but had the SCT in the
>> >> curl geometry.  So you can see that even with TRT in the perfect geometry
>> >> (Iter0) the TRT segments have a PT bias caused by the misalignment between
>> >> the SCT and TRT.
> > 
> > There is a substantial bias in phi0 after 8 iterations. Does this mean that
> > because in the process of curl correction a net rotation is introduced to the
> > entire Si tracker, and therefore one observes this shift w/r/t the truth? (in
> > other words no CoG-like re-centering of the Si was done after alignment)?

Yes this is correct.  It seemed that the inner modules would want to rotate
to correct for the bias while the outer layers would stay relatively fixed.
IF you remember the curl geometry the delta phi was proportional to r. So
the outer modules would be a rotated the most.  The alignment procedure
seemed to love to rotate the inner part of the detector more and I really
don't know why.

I have just thought of way to correct for this with out redoing the trt L1
alignment.  That would be to use the phi from the TRT tracks also as a
pseudo measurement on the track.  This should remove the biases seen here
but I am unsure if it will completely remove them. If we going to use on
track parameter why not another :P. This would be much quicker to accomplish
and I probably could do it Wednesday next week.

\end{verbatim}

From Ben:
\begin{verbatim}
Hi Oleg,

Very sorry for not responding earlier today - I only just saw your p.s. at the bottom of the email. I hope these plots don't come too late for the discussion....

I have managed to locate the folder of plots that appear to correspond with the plot I showed at the Physics week at the start of November last year (see slide 11):
http://indico.cern.ch/getFile.py/access?contribId=3&sessionId=3&resId=0&materialId=slides&confId=41483

This figure is attached, along with the corresponding plot for endcap C and the barrel region. The black is the perfect alignment case, the red the Curl deformation and the blue after the alignment correction. As best I can remember this alignment is produced with a single Level 2 iteration of the GX2 alignment (running on the multimuons) using the additional momentum constraint that you and Pawel derived. The figure is made by running the alignment monitoring over a 20k Zmumu sample - the tracks used are reconstructed using silicon hits only.

I also have plots showing the results after a second iteration, attached with appended "_2ndIter" (here the results were not quite as good).

I am very happy to contribute to the note - unfortunately I will be quite busy this month, trying to get plots approved to be shown at this LHC Alignment workshop in June, but let me know if you need anything and I'll do my best to help.

Cheers, Ben 
\end{verbatim}
******************
\begin{verbatim}
I have put the original Root files here:
~bdcooper/public/RootFilesForOleg

These are the first iteration results. This Root file has a directory structure, the histos you want are here:
IDAlignMon/ResolvedTracks_NoTriggerSelection/TruthComparison/dqopt_barrel
IDAlignMon/ResolvedTracks_NoTriggerSelection/TruthComparison/dqopt_eca
IDAlignMon/ResolvedTracks_NoTriggerSelection/TruthComparison/dqopt_ecc

>
>
> You mention a second iteration: was it done with the same constraint? I mean that the additive bias to the curvature measurement which we assume needs to be re-derived after each iteration, and it would not surprise me that if one took the "old" bias value from the first iteration one would overcorrect and get a deterioration of results. But maybe I am drawing wrong conclusions here?

Right, I am almost certain that you are correct, that the second iteration was done with the same constraint as the first and so we were not surprised to see the result degrade - maybe Pawel can also recall what we did.

\end{verbatim}

